What Exactly Does Guidance Do in Masked Discrete Diffusion Models

We study masked discrete diffusion models with classifier-free guidance (CFG). Assuming no score error nor discretization error, we derive an explicit solution to the guided reverse dynamics, so that how guidance influences the sampling behavior can be precisely characterized. When the full data distribution is a mixture over classes and the goal is to sample from a specific class, guidance amplifies class-specific regions while suppresses regions shared with other classes. This effect depends on the guidance strength $w$ and induces distinct covariance structures in the sampled distribution. Notably, we observe quantitatively different behaviors in $1$D and $2$D. We also show that for large $w$, the decay rate of the total variation ($\mathrm{TV}$) along the reverse dynamics is double-exponential in $w$ for both $1$D and $2$D. These findings highlight the role of guidance, not just in shaping the output distribution, but also in controlling the dynamics of the sampling trajectory. Our theoretical analysis is supported by experiments that illustrate the geometric effects of guidance and its impact on convergence.

==> macro.tex <==
\usepackage{fancyhdr,listings,amsfonts,amsmath,color}
\usepackage[linktocpage,colorlinks,linkcolor=blue,anchorcolor=blue,citecolor=blue,urlcolor=blue,pagebackref]{hyperref}
\usepackage{algorithmicx,algcompatible}
\usepackage[noend]{algpseudocode}

\usepackage{latexsym,amssymb,amsmath,amsfonts,amsthm,xcolor,graphicx, longtable,tabularx}
\RequirePackage[ruled,vlined]{algorithm2e}
\RequirePackage{algpseudocode}
\usepackage{amsmath}
\usepackage{mdframed}
\usepackage{float}
\usepackage{color}
\usepackage{pifont}
\usepackage{listings,amsfonts,amsmath,color,amsthm}
\usepackage{subcaption}
\usepackage{placeins} 
\hypersetup{colorlinks=true,linkcolor=blue}
\usepackage{latexsym,amssymb,amsmath,amsfonts,amsthm,xcolor,graphicx}
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{enumitem,subcaption,ragged2e}
\usepackage{color}
\usepackage{pifont}
\usepackage{amssymb}
\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother
%\usepackage{indentfirst}
\usepackage{multirow}
\usepackage{diagbox}
\usepackage{cancel}
\usepackage{bbm}
\usepackage{xcolor}
\usepackage{mathtools}
\usepackage{natbib,todonotes}
\usepackage{booktabs}

\newcommand{\ye}[1]{{\color{purple}\bf[YE: #1]}}
 {
      \theoremstyle{plain}
      \newtheorem{assumption}{Assumption}[section]
 }
\newcommand\deq{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny d}}}{=}}}
\newcommand{\lv}{\left\lVert}
\newcommand{\rv}{\right\rVert}
\newcommand{\m}{\mathbf}
\newcommand{\ol}{\overline}
\newcommand{\mf}{\mathbf}
\newcommand{\mb}{\mathbb}
\newcommand{\dee}{\mathrm{d}}
\newcommand{\mc}{\mathcal}
\newcommand{\T}{\Tilde}
\newcommand{\e}{\epsilon}
\newcommand{\n}{\nu}
\newcommand{\p}{\pi}
\newcommand{\D}{\mathcal{D}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\bQ}{\Bar{Q}}
\newcommand{\Clow}{C_{\text{Low}}}
\newcommand{\Var}{\text{Var}}
\newcommand{\CPI}{C_{\text{PI}}}
\newcommand{\ora}{\overrightarrow}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\id}{\mathrm{Id}}
\newcommand{\Hessphi}{\text{Hess}\phi^*}
\newcommand{\binner}[2]{\langle {#1}, {#2} \rangle}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\tr}{\mathrm{Tr}}
\newcommand{\Rc}{\mathrm{rc}}
\newcommand{\Sc}{\mathrm{sc}}
\newcommand{\HS}{\mathrm{HS}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand\mmid{\mathbin{\vert}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{question}{Q\hspace{-0.04in}}
\newtheorem{proposition}{Proposition}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
% Alternative Assumption!
\newtheorem{assumptionalt}{Assumption}[assumption]
% New environment
\newenvironment{assumptionp}[1]{
  \renewcommand\theassumptionalt{#1}
  \assumptionalt
}{\endassumptionalt}

\usepackage{mathtools}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\angl{\langle}{\rangle}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\am}[1]{\textbf{\color{purple}[AM: #1]}}
\newcommand{\Xstable}{X_{t}^{(\alpha)}}
\newcommand{\denstable}{p_t^{(\alpha)}}
\usepackage{natbib}
\bibliographystyle{abbrvnat}
\setcitestyle{authoryear,open={(},close={)}} 
\allowdisplaybreaks


\renewcommand*{\backref}[1]{\ifx#1\relax \else Page #1 \fi}
\renewcommand*{\backrefalt}[4]{%
  \ifcase #1 \footnotesize{(Not cited.)}%
  \or        \footnotesize{(Cited on page~#2.)}%
  \else      \footnotesize{(Cited on pages~#2.)}%
  \fi
}


\newcommand{\M}{\mathrm{M}}
\newcommand{\UM}{\mathrm{UM}}
\newcommand{\Softmax}{\mathrm{Softmax}}
\newcommand{\Hess}{\mathrm{Hessian}}
